OPANAS: One-Shot Path Aggregation Network Architecture Search for Object Detection

Recently, neural architecture search (NAS) has been exploited to design feature pyramid networks (FPNs) and achieved promising results for visual object detection. Encouraged by the success, we propose a novel One-Shot Path Aggregation Network Architecture Search (OPANAS) algorithm, which significantly improves both searching efficiency and detection accuracy. Specifically, we first introduce six heterogeneous information paths to build our search space, namely top-down, bottom-up, fusing-splitting, scale-equalizing, skip-connect and none. Second, we propose a novel search space of FPNs, in which each FPN candidate is represented by a densely-connected directed acyclic graph (each node is a feature pyramid and each edge is one of the six heterogeneous information paths). Third, we propose an efficient one-shot search method to find the optimal path aggregation architecture, that is, we first train a super-net and then find the optimal candidate with an evolutionary algorithm. Experimental results demonstrate the efficacy of the proposed OPANAS for object detection: (1) OPANAS is more efficient than state-of-the-art methods (e.g., NAS-FPN and Auto-FPN), at significantly smaller searching cost (e.g., only 4 GPU days on MS-COCO); (2) the optimal architecture found by OPANAS significantly improves main-stream detectors including RetinaNet, Faster R-CNN and Cascade R-CNN, by 2.3-3.2 % mAP comparing to their FPN counterparts; and (3) a new state-of-the-art accuracy-speed trade-off (52.2 % mAP at 7.6 FPS) at smaller training costs than comparable state-of-the-arts. Code will be released at https://github.com/VDIGPKU/OPANAS.

==> chap/experiment_ori.tex <==
\section{Experiments}
\subsection{Implementation Details}

We conduct experiments on \textit{MS-COCO} benchmark \cite{LinMBHPRDZ14} and PASCAL VOC \cite{EveringhamGWWZ10}. 
COCO contains 80 object classes. For COCO, we train on the 118k training images and conduct ablation studies on 5k \texttt{minival} images. We also report the results on the 20k images in \texttt{test-dev} for comparison with SOTA. For evaluation, we adopt the metrics from COCO detection evaluation criteria which is mean Average Precision (mAP) across IoU thresholds from 0.5 to 0.95 with different scales.
%COCO 2017 contains 118k images for training, 5k for evaluation, and 20k for \texttt{test-dev}. 
PASCAL VOC \cite{EveringhamGWWZ10} contains 20 object classes.
For PASCAL VOC, training is performed on the union of VOC 2007 trainval and VOC 2012 trainval (10K images) and evaluation is on VOC 2007 test (4.9K images), mAP scores using IoU at 0.5 is used for evalutation. 
%We only report mAP scores using IoU at 0.5.

\subsubsection{Super-net Training and Sub-net Searching Phase}
We consider a total of $N=5$ intermediate nodes and $K=6$ information paths.
%path types 
for MPOS-FPN super-net training and optimal sub-net searching. 
%The search space has less than $10^{12}$ candidate architectures thanks to the prior information of the hand-designed information paths.
ResNet-50 \cite{HeZRS16} pre-trained on ImageNet \cite{KrizhevskySH12} is used as
our backbone network. During super-net training, we use input-size $800\times 500$ 
%randomly sample $1/5$ from the fully train-set of COCO \cite{LinMBHPRDZ14} with input $800\times 500$ 
to further reduce the search cost. As for PASCOL VOC, the input-size is set to $384\times 384$. We use SGD optimizer with initial learning rate 0.02, momentum 0.9, and $10^{-4}$ as weight decay. We train super-net with 12 epochs with batch size of 16. Additional constraint $\gamma$ is initialized as 1, 
and hyper-parameter $\mathcal{E}$ is $10^{-4}$.
The pruning number $M$ is set to 5. In total, the whole search phase can be finished within 4 days (1 day for super-net training and 3 days for optimal sub-net search) using 1 V100 GPU.

\input{tables/2_table}
\subsubsection{Full Training Phase}
In this phase, we fully train the searched model.
After identifying the optimal sub-net, SGD is performed to train the full model with batch size of 16.
%on 8 GPUs with 2 images on each GPU. 
The initial learning rate is 0.02; $10^{-4}$ as weight decay; 0.9 as momentum. Single-scale training with input $1333\times 800 $ size is trained for 12 epochs, and the learning rate is decreased by 10 at epoch 8 and 11. While multi-scale training (pixel size={$400 \sim 1400$}) is trained for 24 epochs with learning rate decreased by a factor of 0.1 at epoch 16 and 22.
%For evaluation, we adopt the metrics from COCO detection evaluation criteria which is mean Average Precision (mAP) across IoU thresholds from 0.5 to 0.95 with different scales.
%\subsection{Search Results}
\subsection{Results}
The searched optimal MPOS-FPN architecture
is illustrated in Fig. \ref{fig:super-net} (c). 
To demonstrate the effectiveness of our searched architecture which is aggregation of information paths,
we compare it with each path in Tab. \ref{tab:search result}. We choose
the original Faster R-CNN (ResNet50)
as the baseline, and we carefully adjust the channel dimensions of MPOS-FPN and Head, aiming to align the complexity with baseline.
Our searched MPOS-FPN significantly surpasses baseline, 39.6\% vs. 36.4\% in terms of AP with fewer FLOPs/Params (FLOPs 197G vs. 207G, Params 35.5M vs. 41.5M), achieving an effective aggregation and exploration of information paths.
To evaluate the transferability of our MPOS-FPN, we transfer the searched architecture between COCO and VOC, as shown in Tab. \ref{tab:cros-valid}. With the architecture searched
in COCO, our method boosts $2.8\%$ mAP for VOC, $2.9\%$ mAP improvement of VOC training and COCO test, 
%vice versa,
further demonstrating
the effectiveness of our method.
\input{tables/4_table}


\subsubsection{Model Transferability}%Model Extension}
To verify the transferability of the searched MPOS-FPN architecture, we adapt this architecture
on the top of RetinaNet \cite{LinGGHD17} and Cascade RCNN \cite{FelzenszwalbGM10} in Tab. \ref{tab:modelextention}. Under the same training strategy with baseline, we obtain a lighter model {with better performance on each detector (\textit{e.g,} improving RetinaNet by 2.3$\%$ mAP with 13$\%$ GFlops decreasing, and improving Cascade RCNN by 2.5$\%$ mAP with 27$\%$ parameter amount decreasing)}, achieving a better  
accuracy-efficiency
trade-off. 
%All these results demonstrate the effectiveness of the searched MPOS-FPN.

\subsubsection{Comparison with SOTA}
We further conduct comparison with state-of-the-art detectors,
including hand-crafted \cite{DBLP:journals/corr/abs-1911-09070}, and NAS based ones (\cite{DBLP:conf/cvpr/GuoHWZYW0020, DBLP:journals/corr/abs-1911-09929,  DBLP:conf/cvpr/GhiasiLL19,  DBLP:conf/cvpr/WangGCWTSZ20, DBLP:conf/cvpr/DuLJGTCLS20,  Xu_2019_ICCV, DBLP:conf/nips/ChenYZMXS19}).
%including hand-crafted EfficientDet \cite{DBLP:journals/corr/abs-1911-09070}, and NAS based ones (Hit-Detector \cite{DBLP:conf/cvpr/GuoHWZYW0020}, SM-NAS \cite{DBLP:journals/corr/abs-1911-09929}, NAS-FPN \cite{DBLP:conf/cvpr/GhiasiLL19}, NAS-FCOS \cite{DBLP:conf/cvpr/WangGCWTSZ20}, SpineNet \cite{DBLP:conf/cvpr/DuLJGTCLS20}, Auto-FPN \cite{Xu_2019_ICCV} and DetNAS \cite{DBLP:conf/nips/ChenYZMXS19}). %It’s worth noting that, 
Note that these methods search different components of detectors. Specifically, SM-NAS searches 
the overall architecture of Cascade RCNN, NAS-FPN searches 
the neck architecture, and Auto-FPN searches  
the architectures of both neck and detection head. 
As shown in Tab. \ref{tab:comparenas}, comparing with representative results achieved by these SOTA methods, our method achieves better or very competitive results in terms of parameter amount, computation complexity, accuracy, and inference speed. 
Our method can search  the best neck architecture more efficiently. {With only 4 V100 GPU days search, our searched MPOS-FPN equipped with Cascade R-CNN Res2Net101-DCN outperforms SpineNet by 0.4 $\%$ mAP while using only 1/2 FLops with significantly smaller search cost (700$\times \#$TPUs) .vs 4 V100 GPUs}, achieving 52.5 $\%$ mAP on COCO. This demonstrate %proves 
the effectiveness of our carefully designed search space 
and the efficiency of the search algorithm.

\subsection{Ablation Study}
\begin{figure}
	\centering
	\begin{minipage}{\linewidth}
		\centering
		\subfloat[\centering mmAP]{{\includegraphics[width=.44\linewidth]{imgs/constrain_ap} }}
		\qquad
		\subfloat[\centering Loss]{{\includegraphics[width=.44\linewidth]{imgs/constrain_loss} }}
		\qquad
		\subfloat[\centering search process]{{\includegraphics[width=\linewidth]{imgs/ea} }}
		\qquad
		
		\caption{Comparison of training MPOS-FPN super-net w or w/o additional constraint. mmAP denotes the mean mAP of random sampled 50 sub-nets from current epoch.}%
		\label{fig:additional constraint}%
	\end{minipage}
		\vspace{-1em}

\end{figure}
\subsubsection{Edge Importance Weight}
To show the effectiveness of the edge importance weight $\gamma$ in Eq. (\ref{eq:gamma}) %5additional constraint comment: please specify this? 
%which variable in which equation
, we illustrate the training and searching process of the super-net of MPOS-FPN with fair sampling. As illustrated in Fig. \ref{fig:additional constraint}, additional constraint can accelerate the convergence of super-net training and make this
training more adequate. This proves that distinguishing the importance of different edges  is effective for multi-path super-net training.

\subsubsection{Correlation Analysis}
Recently, the effectiveness of weight sharing based NAS methods
is questioned because of the lack of (1) 
fair comparison on the same search space and (2) adequate analysis on the correlation between the super-net performance and the stand-alone sub-net model performance \cite{DBLP:journals/corr/abs-1904-00420}. Here we adopt Kendall Tau \cite{correlation} to measure the correlation of model ranking obtained from super-net. Specifically, we randomly sample 15 sub-nets from the trained super-net, and conduct full train to evaluate their performance. 
%DAG models from all the searched structures trained on COCO with batch size 16. 
%Since full training on COCO is time-consuming, we reduce the epoch number to 9 and set the input size as $800 \times 500$. 
%The model is then evaluated on the COCO 2017 validation set. 
In Tab. \ref{tab:correlation}, when changing from single-path used by SPOS \cite{DBLP:journals/corr/abs-1904-00420} to our multi-path, there is a drop in correlation. %When adopted with
When we adopt fair sampling and additional constrain, we achieve much high correlation value: 0.6145   vs. 0.3584 (without fair sampling), showing that  our method has higher correlation between super-net and sub-net training. 
%\hu{the result is getting more credible and comparable with correlation $tau$ improves by 0.2561 into 0.6145. comments: proof?} 
%Poor and well-performing architectures can be distinguished by the super-net weight-sharing training. \hu{comments: this conclusion is not reasonable, at least not straightforward}

\subsubsection{Comparison of More NAS Baselines}
We further compare our method with more popular NAS methods using the same search space %add more NAS baselines 
to validate
the efficacy of our method: a) Random Search: We randomly sample 15 architectures from the current search space and conduct full train under the same training setting in our experiments; b) SPOS: we train the single-path one-shot FPN super-net and perform EA search strategy following \cite{DBLP:journals/corr/abs-1904-00420}. c) DARTS: it is a very popular differentiable NAS method; %we \hu{resemble the search space comments: what do you mean here} as DARTS \cite{DBLP:conf/iclr/LiuSY19}, by adjusting the entry-degree of the parameterized information paths of each intermediate node to no more than 2. 
d) Fair DARTS: similar search strategy to DARTS expect %but with 
softmax relaxation and zero-one loss \cite{DBLP:conf/cvpr/JiangXZLL20}. Tab. \ref{tab:nasabla} demonstrates the effectiveness of our method. Compared with other NAS methods, our method can search a better architecture with less or comparable time. This proves the effectiveness of our super-net training and optimal sub-net search strategy.
%that gradient methods are not suitable for our MPOS-FPN search space. We think this is because our 2 parameter-free information paths affect the gradient calculation of the parameterized architecture. 
\input{tables/3_table}
\input{tables/6_table}


